FREED++: Improving RL Agents for Fragment-Based Molecule Generation by Thorough Reproduction

A rational design of new therapeutic drugs aims to find a molecular structure with desired biological functionality, e.g., an ability to activate or suppress a specific protein via binding to it. Molecular docking is a common technique for evaluating protein-molecule interactions. Recently, Reinforcement Learning (RL) has emerged as a promising approach to generating molecules with the docking score (DS) as a reward. In this work, we reproduce, scrutinize and improve the recent RL model for molecule generation called FREED (arXiv:2110.01219). Extensive evaluation of the proposed method reveals several limitations and challenges despite the outstanding results reported for three target proteins. Our contributions include fixing numerous implementation bugs and simplifying the model while increasing its quality, significantly extending experiments, and conducting an accurate comparison with current state-of-the-art methods for protein-conditioned molecule generation. We show that the resulting fixed model is capable of producing molecules with superior docking scores compared to alternative approaches.

==> figs/5.1/Baselines_Metrics.tex <==
\begin{tabular}{llllllllll}
\toprule
     &      &        valid &       unique &                   LogP &          QED &                    SA &                 PAINS &            SureChEMBL &                 Glaxo \\
protein & name &              &              &                        &              &                       &                       &                       &                       \\
\midrule
\hline
fa7 & CombGen &  1.00 ± 0.00 &  0.98 ± 0.00 &            3.04 ± 0.01 &  0.65 ± 0.00 &           2.70 ± 0.00 &           0.99 ± 0.00 &           0.90 ± 0.00 &           0.98 ± 0.00 \\
     & MolDQN &  1.00 ± 0.00 &  0.19 ± 0.01 &   \textbf{-3.70 ± 0.26} &  0.08 ± 0.00 &           6.65 ± 0.24 &           0.72 ± 0.01 &   \textbf{0.00 ± 0.00} &   \textbf{0.41 ± 0.35} \\
     & REINVENT &  0.99 ± 0.00 &  0.99 ± 0.00 &            6.09 ± 1.44 &  0.34 ± 0.05 &   \textbf{2.29 ± 0.04} &           0.99 ± 0.00 &           0.60 ± 0.15 &           0.87 ± 0.19 \\
     & Pocket2Mol &  1.00 ± 0.00 &  1.00 ± 0.00 &            3.96 ± 0.18 &  0.53 ± 0.02 &           3.20 ± 0.26 &           0.89 ± 0.14 &           0.49 ± 0.19 &           0.98 ± 0.00 \\
     & FREED &  1.00 ± 0.00 &  0.43 ± 0.40 &            4.82 ± 0.76 &  0.48 ± 0.07 &           4.44 ± 0.23 &           0.97 ± 0.02 &           0.77 ± 0.24 &           0.74 ± 0.23 \\
     & FFREED &  1.00 ± 0.00 &  0.53 ± 0.12 &            9.09 ± 0.18 &  0.17 ± 0.00 &           4.39 ± 0.28 &   \textbf{0.16 ± 0.08} &           0.96 ± 0.01 &           0.99 ± 0.00 \\
     & FREED++ &  1.00 ± 0.00 &  0.76 ± 0.05 &            9.05 ± 0.35 &  0.19 ± 0.02 &           4.13 ± 0.12 &           0.33 ± 0.21 &           0.97 ± 0.00 &           0.99 ± 0.00 \\
     & DUDE &     1.00 ± - &     1.00 ± - &               3.99 ± - &     0.22 ± - &              2.87 ± - &              0.98 ± - &              0.15 ± - &              0.98 ± - \\
\hline
parp1 & CombGen &  1.00 ± 0.00 &  0.98 ± 0.00 &            3.04 ± 0.01 &  0.65 ± 0.00 &           2.70 ± 0.00 &           0.99 ± 0.00 &           0.90 ± 0.00 &           0.98 ± 0.00 \\
     & MolDQN &  1.00 ± 0.00 &  0.22 ± 0.02 &   \textbf{-1.33 ± 0.32} &  0.15 ± 0.03 &           7.02 ± 0.04 &           0.60 ± 0.27 &   \textbf{0.00 ± 0.00} &   \textbf{0.41 ± 0.17} \\
     & REINVENT &  0.98 ± 0.00 &  0.98 ± 0.02 &            6.88 ± 0.14 &  0.32 ± 0.03 &   \textbf{2.26 ± 0.18} &           0.99 ± 0.00 &           0.68 ± 0.19 &           0.95 ± 0.02 \\
     & Pocket2Mol &  1.00 ± 0.00 &  1.00 ± 0.00 &            4.05 ± 0.10 &  0.48 ± 0.01 &           4.24 ± 0.33 &           0.92 ± 0.01 &           0.80 ± 0.11 &           0.93 ± 0.07 \\
     & FREED &  1.00 ± 0.00 &  0.33 ± 0.32 &            5.56 ± 2.30 &  0.41 ± 0.09 &           4.37 ± 0.69 &           0.95 ± 0.02 &           0.89 ± 0.12 &           0.91 ± 0.09 \\
     & FFREED &  1.00 ± 0.00 &  0.58 ± 0.09 &            8.66 ± 0.30 &  0.22 ± 0.00 &           3.80 ± 0.30 &           0.68 ± 0.33 &           0.96 ± 0.00 &           0.98 ± 0.00 \\
     & FREED++ &  1.00 ± 0.00 &  0.71 ± 0.06 &            9.18 ± 0.32 &  0.21 ± 0.00 &           3.88 ± 0.26 &   \textbf{0.45 ± 0.27} &           0.97 ± 0.00 &           0.98 ± 0.01 \\
     & DUDE &     1.00 ± - &     1.00 ± - &               2.47 ± - &     0.67 ± - &              2.66 ± - &              0.98 ± - &              0.96 ± - &              0.99 ± - \\
\hline
5ht1b & CombGen &  1.00 ± 0.00 &  0.98 ± 0.00 &            3.04 ± 0.01 &  0.65 ± 0.00 &           2.70 ± 0.00 &           0.99 ± 0.00 &           0.90 ± 0.00 &           0.98 ± 0.00 \\
     & MolDQN &  1.00 ± 0.00 &  0.20 ± 0.03 &   \textbf{-2.67 ± 0.63} &  0.09 ± 0.03 &           6.81 ± 0.06 &   \textbf{0.58 ± 0.17} &   \textbf{0.01 ± 0.01} &   \textbf{0.29 ± 0.22} \\
     & REINVENT &  0.98 ± 0.01 &  0.99 ± 0.01 &            6.02 ± 0.57 &  0.44 ± 0.07 &   \textbf{2.20 ± 0.16} &           0.96 ± 0.04 &           0.77 ± 0.17 &           0.94 ± 0.05 \\
     & Pocket2Mol &  1.00 ± 0.00 &  1.00 ± 0.00 &            5.34 ± 0.54 &  0.41 ± 0.04 &           4.86 ± 0.32 &           0.98 ± 0.01 &           0.82 ± 0.04 &           0.94 ± 0.05 \\
     & FREED &  1.00 ± 0.00 &  0.21 ± 0.21 &            5.28 ± 2.66 &  0.33 ± 0.08 &           4.81 ± 0.97 &           0.63 ± 0.54 &           0.56 ± 0.50 &           0.60 ± 0.53 \\
     & FFREED &  1.00 ± 0.00 &  0.45 ± 0.11 &            7.40 ± 0.31 &  0.33 ± 0.01 &           2.62 ± 0.36 &           0.99 ± 0.00 &           0.93 ± 0.02 &           0.98 ± 0.00 \\
     & FREED++ &  1.00 ± 0.00 &  0.45 ± 0.07 &            7.56 ± 0.08 &  0.36 ± 0.03 &           3.08 ± 0.14 &           0.97 ± 0.00 &           0.89 ± 0.04 &           0.99 ± 0.00 \\
     & DUDE &     1.00 ± - &     1.00 ± - &               3.47 ± - &     0.68 ± - &              2.60 ± - &              1.00 ± - &              0.84 ± - &              0.98 ± - \\
\hline
fkb1a & CombGen &  1.00 ± 0.00 &  0.98 ± 0.00 &            3.04 ± 0.01 &  0.65 ± 0.00 &           2.70 ± 0.00 &           0.99 ± 0.00 &           0.90 ± 0.00 &           0.98 ± 0.00 \\
     & MolDQN &  1.00 ± 0.00 &  0.18 ± 0.03 &   \textbf{-2.89 ± 0.40} &  0.24 ± 0.07 &           6.91 ± 0.15 &   \textbf{0.88 ± 0.10} &   \textbf{0.06 ± 0.01} &   \textbf{0.36 ± 0.32} \\
     & REINVENT &  0.99 ± 0.00 &  0.93 ± 0.03 &            5.45 ± 0.71 &  0.54 ± 0.07 &   \textbf{2.64 ± 0.21} &           0.99 ± 0.00 &           0.72 ± 0.22 &           0.94 ± 0.04 \\
     & Pocket2Mol &  1.00 ± 0.00 &  1.00 ± 0.00 &            4.40 ± 0.79 &  0.42 ± 0.02 &           3.91 ± 0.14 &           0.96 ± 0.00 &           0.65 ± 0.13 &           0.96 ± 0.03 \\
     & FREED &  1.00 ± 0.00 &  0.44 ± 0.32 &            4.53 ± 1.28 &  0.43 ± 0.04 &           3.98 ± 0.72 &           0.89 ± 0.03 &           0.55 ± 0.09 &           0.67 ± 0.38 \\
     & FFREED &  1.00 ± 0.00 &  0.36 ± 0.14 &            5.82 ± 0.47 &  0.58 ± 0.04 &           3.82 ± 0.22 &           0.97 ± 0.01 &           0.76 ± 0.01 &           0.96 ± 0.01 \\
     & FREED++ &  1.00 ± 0.00 &  0.30 ± 0.03 &            6.01 ± 0.17 &  0.59 ± 0.01 &           4.18 ± 0.13 &           0.98 ± 0.00 &           0.78 ± 0.00 &           0.93 ± 0.03 \\
     & DUDE &     1.00 ± - &     1.00 ± - &               3.88 ± - &     0.44 ± - &              3.39 ± - &              1.00 ± - &              0.84 ± - &              0.98 ± - \\
\hline
abl1 & CombGen &  1.00 ± 0.00 &  0.98 ± 0.00 &            3.04 ± 0.01 &  0.65 ± 0.00 &           2.70 ± 0.00 &           0.99 ± 0.00 &           0.90 ± 0.00 &           0.98 ± 0.00 \\
     & MolDQN &  1.00 ± 0.00 &  0.16 ± 0.02 &    \textbf{0.09 ± 0.50} &  0.23 ± 0.10 &           6.30 ± 0.14 &   \textbf{0.58 ± 0.12} &   \textbf{0.08 ± 0.07} &   \textbf{0.45 ± 0.30} \\
     & REINVENT &  0.99 ± 0.00 &  0.85 ± 0.03 &            5.80 ± 1.31 &  0.41 ± 0.12 &           2.55 ± 0.09 &           0.96 ± 0.04 &           0.30 ± 0.15 &           0.97 ± 0.02 \\
     & Pocket2Mol &  1.00 ± 0.00 &  1.00 ± 0.00 &            3.69 ± 0.34 &  0.38 ± 0.04 &           3.97 ± 0.23 &           0.82 ± 0.10 &           0.68 ± 0.04 &           0.97 ± 0.03 \\
     & FREED &  1.00 ± 0.00 &  0.24 ± 0.23 &            3.69 ± 1.38 &  0.41 ± 0.11 &           4.15 ± 1.45 &           0.92 ± 0.07 &           0.83 ± 0.16 &           0.89 ± 0.14 \\
     & FFREED &  1.00 ± 0.00 &  0.39 ± 0.12 &            5.67 ± 0.12 &  0.61 ± 0.00 &           2.32 ± 0.05 &           0.98 ± 0.01 &           0.51 ± 0.30 &           0.97 ± 0.01 \\
     & FREED++ &  1.00 ± 0.00 &  0.34 ± 0.02 &            5.57 ± 0.01 &  0.61 ± 0.02 &   \textbf{2.19 ± 0.12} &           0.99 ± 0.00 &           0.73 ± 0.08 &           0.97 ± 0.02 \\
     & DUDE &     1.00 ± - &     1.00 ± - &               4.71 ± - &     0.43 ± - &              2.77 ± - &              0.97 ± - &              0.79 ± - &              0.96 ± - \\
\hline
usp7 & CombGen &  1.00 ± 0.00 &  0.98 ± 0.00 &            3.04 ± 0.01 &  0.65 ± 0.00 &           2.70 ± 0.00 &           0.99 ± 0.00 &           0.90 ± 0.00 &           0.98 ± 0.00 \\
     & MolDQN &  1.00 ± 0.00 &  0.21 ± 0.03 &   \textbf{-1.83 ± 0.72} &  0.18 ± 0.08 &           6.52 ± 0.16 &   \textbf{0.58 ± 0.26} &   \textbf{0.04 ± 0.03} &   \textbf{0.46 ± 0.37} \\
     & REINVENT &  0.98 ± 0.00 &  0.99 ± 0.00 &            5.63 ± 1.11 &  0.42 ± 0.09 &   \textbf{2.26 ± 0.10} &           0.98 ± 0.01 &           0.66 ± 0.17 &           0.88 ± 0.13 \\
     & Pocket2Mol &  1.00 ± 0.00 &  1.00 ± 0.00 &            3.05 ± 0.05 &  0.56 ± 0.02 &           3.84 ± 0.10 &           0.95 ± 0.04 &           0.85 ± 0.04 &           0.98 ± 0.00 \\
     & FREED &  1.00 ± 0.00 &  0.10 ± 0.07 &            6.22 ± 1.75 &  0.45 ± 0.08 &           4.38 ± 0.87 &           0.99 ± 0.00 &           0.90 ± 0.06 &           0.93 ± 0.06 \\
     & FFREED &  1.00 ± 0.00 &  0.66 ± 0.01 &            7.32 ± 0.41 &  0.34 ± 0.02 &           3.74 ± 0.12 &           0.66 ± 0.28 &           0.90 ± 0.05 &           0.98 ± 0.01 \\
     & FREED++ &  1.00 ± 0.00 &  0.64 ± 0.07 &            8.07 ± 0.30 &  0.28 ± 0.00 &           2.70 ± 0.08 &           0.94 ± 0.04 &           0.91 ± 0.04 &           0.99 ± 0.00 \\
     & DUDE &     1.00 ± - &     1.00 ± - &               4.01 ± - &     0.55 ± - &              3.64 ± - &              1.00 ± - &              0.97 ± - &              0.72 ± - \\
\bottomrule
\end{tabular}


==> figs/5.3/FilteredFragments_DS.tex <==
\begin{tabular}{llllllllll}
\toprule
method & library   &       unique ($\uparrow$) &                 Avg DS ($\uparrow$) &                 Max DS ($\uparrow$) &               Top-5 DS ($\uparrow$) &                 PAINS ($\uparrow$) &            SureChEMBL ($\uparrow$) &                 Glaxo ($\uparrow$) \\
\midrule
\hline
FREED++ & filtered &  0.64 ± 0.07 &   \textbf{11.37 ± 0.23} &           13.76 ± 0.40 &           13.27 ± 0.23 &           0.99 ± 0.00 &           0.92 ± 0.03 &           0.99 ± 0.00 \\
 & vanilla &  0.64 ± 0.07 &            9.66 ± 3.28 &   \textbf{14.16 ± 0.47} &   \textbf{13.30 ± 0.13} &           0.94 ± 0.04 &           0.91 ± 0.04 &           0.99 ± 0.00 \\
FREED & filtered &  0.14 ± 0.23 &            3.22 ± 5.14 &            5.13 ± 6.76 &            4.05 ± 6.57 &   \textbf{1.00 ± 0.00} &   \textbf{0.99 ± 0.01} &   \textbf{1.00 ± 0.00} \\
 & vanilla &  0.10 ± 0.07 &            8.58 ± 1.02 &           11.36 ± 0.98 &           11.12 ± 0.88 &           0.99 ± 0.00 &           0.90 ± 0.06 &           0.93 ± 0.06 \\
\bottomrule
\end{tabular}


==> figs/5.3/FilteredFragments_DS_1.tex <==
\begin{tabular}{llllllllll}
\toprule
method & library   &       unique ($\uparrow$) &                 Avg DS ($\uparrow$) &                 Max DS ($\uparrow$) &               Top-5 DS ($\uparrow$)\\
\midrule
\hline
FREED++ & filtered &  0.64 ± 0.07 &   \textbf{11.37 ± 0.23} &           13.76 ± 0.40 &           13.27 ± 0.23 \\
 & vanilla &  0.64 ± 0.07 &            9.66 ± 3.28 &   \textbf{14.16 ± 0.47} &   \textbf{13.30 ± 0.13} \\
FREED & filtered &  0.14 ± 0.23 &            3.22 ± 5.14 &            5.13 ± 6.76 &            4.05 ± 6.57 \\
 & vanilla &  0.10 ± 0.07 &            8.58 ± 1.02 &           11.36 ± 0.98 &           11.12 ± 0.88 \\
\bottomrule
\end{tabular}

